Rethinking FID: Towards a Better Evaluation Metric for Image Generation

As with many machine learning problems, the progress of image generation methods hinges on good evaluation metrics. One of the most popular is the Frechet Inception Distance (FID). FID estimates the distance between a distribution of Inception-v3 features of real images, and those of images generated by the algorithm. We highlight important drawbacks of FID: Inception's poor representation of the rich and varied content generated by modern text-to-image models, incorrect normality assumptions, and poor sample complexity. We call for a reevaluation of FID's use as the primary quality metric for generated images. We empirically demonstrate that FID contradicts human raters, it does not reflect gradual improvement of iterative text-to-image models, it does not capture distortion levels, and that it produces inconsistent results when varying the sample size. We also propose an alternative new metric, CMMD, based on richer CLIP embeddings and the maximum mean discrepancy distance with the Gaussian RBF kernel. It is an unbiased estimator that does not make any assumptions on the probability distribution of the embeddings and is sample efficient. Through extensive experiments and analysis, we demonstrate that FID-based evaluations of text-to-image models may be unreliable, and that CMMD offers a more robust and reliable assessment of image quality.

==> 03_background.tex <==

\section{Background}

\subsection{Frechet Inception Distance} 

F\'rechet Inception Distance (FID) is used to measure the discrepancy between two image sets. Usually one set of images are real (for example, from the COCO dataset) and the other set is generated using the text-to-image model to be evaluated. To this end, Inception V3 embeddings~\cite{SzegedyVISW15} are visual features from the real and the generated images using the Inception V3 model pretrained on ImageNet. Let $(\mu, \Sigma)$ and $(\mu', \Sigma')$ denote the pair of mean and covariance matrices computed on the visual features from real and generated data, respectively. We compute F\'rechet Inception Distance (FID) as follows:
\begin{equation}
    \operatorname{FID}(\mathcal{I}, \mathcal{I}') = \|\mu - \mu'\|^2_2 + \operatorname{Tr}(\Sigma + \Sigma' - 2(\Sigma\Sigma')^{\frac{1}{2}})
\end{equation}

\subsection{Maximum Mean Discrepancy}
Maximum mean discrepancy is a distribution-free metric to compare two distance. It was originally developed as a part of a two-sample statistical test to determine whether two data samples came from the same distribution. However, the MMD metric, calculated in this test can be use to measure how far two distributions are.

\begin{eqnarray}
    \operatorname{MMD}(X,Y) = \frac{1}{m(m-1)}\sum_{i \ne j}^m k(x_i,x_j) \nonumber \\
    + \frac{1}{n(n-1)}\sum_{i \ne j}^m k(y_i,y_j) \nonumber \\
    - \frac{2}{mn}\sum_{i=1}^m\sum_{j=1}^n k(x_i, y_j)
\end{eqnarray}



